MAMDR: A Model Agnostic Learning Method for Multi-Domain Recommendation

Large-scale e-commercial platforms in the real-world usually contain various recommendation scenarios (domains) to meet demands of diverse customer groups. Multi-Domain Recommendation (MDR), which aims to jointly improve recommendations on all domains and easily scales to thousands of domains, has attracted increasing attention from practitioners and researchers. Existing MDR methods usually employ a shared structure and several specific components to respectively leverage reusable features and domain-specific information. However, data distribution differs across domains, making it challenging to develop a general model that can be applied to all circumstances. Additionally, during training, shared parameters often suffer from the domain conflict while specific parameters are inclined to overfitting on data sparsity domains. we first present a scalable MDR platform served in Taobao that enables to provide services for thousands of domains without specialists involved. To address the problems of MDR methods, we propose a novel model agnostic learning framework, namely MAMDR, for the multi-domain recommendation. Specifically, we first propose a Domain Negotiation (DN) strategy to alleviate the conflict between domains. Then, we develop a Domain Regularization (DR) to improve the generalizability of specific parameters by learning from other domains. We integrate these components into a unified framework and present MAMDR, which can be applied to any model structure to perform multi-domain recommendation. Finally, we present a large-scale implementation of MAMDR in the Taobao application and construct various public MDR benchmark datasets which can be used for following studies. Extensive experiments on both benchmark datasets and industry datasets demonstrate the effectiveness and generalizability of MAMDR.

==> prelimiany.tex <==


\section{Preliminary}

\subsection{Multi-Domain Recommendation and Applications}\label{sec:app}
Multi-Domain Recommendation (MDR) \cite{zhu2021cross} aims to design a system that recommends a group of items to a set of users from multiple domains. The recommender system satisfies diverse user demands and provides personalized experiences under each domain, meanwhile, it can be easily scaled to new domains. 

The Multi-Domain Recommender system (MDR system) served in Taobao is illustrated in Figure \ref{fig:framework}. In our applications, we need to provide services for thousands of different domains, where some of which have limited training data. In training, the recommender model is optimized using user-item interaction histories parsed from the user logs. The interaction histories are collected from different domains. Different domains could share overlapping users/items. Thus, we maintain a global feature storage for all users/items and shared model parameters to server for all domains. We also design specific parameters to provide customized recommendations under each domain. A new domain can be easily added to the system by providing the corresponding users/items. The system would automatically increase specific parameters for this new domain.
However, how to incorporate the shared and specific components together while optimizing them under all domains remains a significant challenge in Multi-Domain Recommendation. The problem of Multi-Domain Recommendation can be defined as:
%MDR simultaneously uses information from all domains to extract common features and consider domain distinctions to improve recommendation results of all domains, which can be defined as follows:

\begin{definition}[\textbf{Multi-Domain Recommendation}]
Given $n$ different domains $\mathcal{D}=\{D^1,\cdots,D^n\}$, each domain $D^i = \{U^i, V^i, T^i\}$ includes a set of users $u \in U^i$ and items $v \in V^i$, where users and items could overlap across domains. The $T^i$ denotes a set of user-item interaction histories $(u,v,y)\in T^i$, where $y\in\{1,0\}$ indicates whether user $u$ clicked item $v$ or not. Thus, Multi-Domain Recommendation aims to use interaction histories of all domains $\mathcal{T}=\{T^1,\cdots T^n\}$ to train a model with parameter $\Theta$ that could recommend interesting items for users in all domains. 

As we discussed in the section \ref{sec:introduction}, some MDR methods split the model parameters $\Theta$ into a set of shared parameters $\theta^S$ and a set of domain-specific parameters $\{\theta^i| i \in [1,n]\}$. The $\theta^S$ are optimized by data from all domains to capture multi-domain features, and the $\theta^i$ is updated on specific domain to capture distinction. Thus, the objective function of MDR can be further formulated as:
    \begin{equation}
        % \setlength\abovedisplayskip{1pt}%shrink space
        % \setlength\belowdisplayskip{1pt}
        \mathcal{O}_M = \min_{\Theta=\{\theta^S,\theta^i\}} \sum_{i=1}^n L(\theta^S,T^i) + L(\theta^i,T^i),
        \label{eq:objective_specific}
    \end{equation}
    where $\theta^S$ are optimized by data from all domains, and $\theta_i$ are only optimized in corresponding domain. 
\end{definition}

\subsection{Domain Conflict}\label{sec:conflict}


\begin{figure}[]
    \centering
    \includegraphics[trim=0 0.5cm 0.8cm 0cm,clip,width=0.5\columnwidth]{figures/domain_conflict.pdf}
    \caption{The illustration of domain conflict. The conflict happens when the inner-product of gradients from different domains is negative.}
    \label{fig:domain_conflict}
\end{figure}

Directly optimizing equations \ref{eq:objective_specific} may deteriorate the recommendation performance. A primary cause for this phenomena is known as domain conflict, which is shown in the Figure \ref{fig:domain_conflict}.
%
For parameters optimized across domains, the gradient from each domain $D^i$ is denoted as $g_i = \bigtriangledown L(\Theta,T^i)$. The $\Theta$ are optimized following the direction of $g_i$, i.e., $\Theta \leftarrow  \Theta - \alpha \cdot g_i$, where $\alpha$ is the learning rate. However, the gradients from different domains may conflict with each other when they point to dissimilar directions. This dissimilarity could be represented by the inner-product between gradients. Thus, the conflict happens when the inner-product of gradients from different domains is negative, i.e., $\langle g_i, g_j\rangle < 0$, where $\langle\cdot,\cdot\rangle$ denotes the inner-product between two gradients. As observed by previous research \cite{yu2020gradient,liu2021conflict}, this conflict will impair the optimization and lead parameters to stay at a compromise point at the loss landscape, which also results in poor recommendation results.




% 现有方法是怎么解决梯度冲突的？有什么问题。
\subsection{Prior Attempts and Limitations}\label{sec:limit}
Some research efforts have been made to solve the domain conflict. In the area of MTL, Alex et al. \cite{kendall2018multi} utilize a learned weighted loss to balance the gradients from different domains. PCGrad \cite{yu2020gradient} relieves the conflict by projecting the gradient into the normal plane of others. In the area of meta-learning, the conflicts of gradients could be averse by projecting them into a common space \cite{flennerhag2019meta} or minimizing the inner-product of them \cite{li2018learning}.

% 现有的拆分参数方法又有啥问题：主导 & 过拟合
However, MTL methods that manipulate gradients could face the convergence problem and stay at a sub-optimal point of the loss landscape \cite{liu2021conflict}. Meanwhile, meta-learning frameworks are originally proposed to apply in unseen domains, which might not fit existing domains' data well. Besides, the above methods are either required to modify the model structure or lack scalability for large MDR. Despite some MDR methods using domain-specific parameters, their share parameters $\theta^S$ still suffer the aforementioned problems. Besides, the uses of specific parameters also meet the overfitting problem when the domain data is insufficient. 

Related to MDR, cross-domain recommendation (CDR) aims to improve the performance of the target domain with the help of auxiliary domains \cite{khan2017cross,loni2014cross,hu2018conet,du2019sequential,liu2021leveraging}. By treating each domain as the target domain and transferring knowledge from each auxiliary domain, CDR methods can be adapted to MDR problems. However, it requires a $O(n^2)$ complexity, which is unacceptable for large-scale applications. We can transfer from multiple domains at a time to reduce complexity, but it also introduces the domain conflict problem.

Thus, in \ourmethod, we introduce the Domain Negotiation (DN) and Domain Regularization (DR) strategies to solve the aforementioned challenges in a linear time complexity.

